Unsupervised Extractive Summarization using Pointwise Mutual Information

Unsupervised approaches to extractive summarization usually rely on a notion of sentence importance defined by the semantic similarity between a sentence and the document. We propose new metrics of relevance and redundancy using pointwise mutual information (PMI) between sentences, which can be easily computed by a pre-trained language model. Intuitively, a relevant sentence allows readers to infer the document content (high PMI with the document), and a redundant sentence can be inferred from the summary (high PMI with the summary). We then develop a greedy sentence selection algorithm to maximize relevance and minimize redundancy of extracted sentences. We show that our method outperforms similarity-based methods on datasets in a range of domains including news, medical journal articles, and personal anecdotes.

==> problemsetup.tex <==
\section{Problem Setup}
\label{sec:problemsetup}

Given a set of documents $P$ of size $N$, the objective of document summarization is to shorten each document $P_i \; \forall \: i \:  \epsilon \{1, ... ,N\} $ to a corresponding summary $S_i$.\\

Specifically we perform extractive summarization at the sentence level. Given a document $P_i$ that consists of sentences, $s_j \; \forall \: j \: \epsilon \{1, ... ,n\}$, the objective is to yield a summary $S_i$ that is the subset of sentences $s$ selected as per the relevance and redundancy criterea as detailed in Section \ref{sec:approach}.\\

\hh{Also need to explain what \emph{unsupervised} summarization is: what's the input and output of our algorithm.}

